Exact Byte-Level Probabilities from Tokenized Language Models for FIM-Tasks and Model Ensembles

Tokenization is associated with many poorly understood shortcomings in language models (LMs), yet remains an important component for long sequence scaling purposes. This work studies how tokenization impacts model performance by analyzing and comparing the stochastic behavior of tokenized models with their byte-level, or token-free, counterparts. We discover that, even when the two models are statistically equivalent, their predictive distributions over the next byte can be substantially different, a phenomenon we term as ``tokenization bias''. To fully characterize this phenomenon, we introduce the Byte-Token Representation Lemma, a framework that establishes a mapping between the learned token distribution and its equivalent byte-level distribution. From this result, we develop a next-byte sampling algorithm that eliminates tokenization bias without requiring further training or optimization. In other words, this enables zero-shot conversion of tokenized LMs into statistically equivalent token-free ones. We demonstrate its broad applicability with two use cases: fill-in-the-middle (FIM) tasks and model ensembles. In FIM tasks where input prompts may terminate mid-token, leading to out-of-distribution tokenization, our method mitigates performance degradation and achieves 18% improvement in FIM coding benchmarks, while consistently outperforming the standard token healing fix. For model ensembles where each model employs a distinct vocabulary, our approach enables seamless integration, resulting in improved performance up to 3.7% over individual models across various standard baselines in reasoning, knowledge, and coding. Code is available at: https://github.com/facebookresearch/Exact-Byte-Level-Probabilities-from-Tokenized-LMs

==> contents/markov_chain_original.tex <==
%\documentclass{report}
%\usepackage{tikz}
%\usetikzlibrary{shapes,arrows,positioning}
%\usetikzlibrary{automata,arrows,positioning,calc}
%\usetikzlibrary{arrows.meta, automata,
%                positioning,
%                quotes}
%\usepackage{amsmath}

%\begin{document}

\begin{figure*}[t]
    \centering
    \vspace{-25pt}
    \begin{tikzpicture}[->, >=stealth', auto, semithick, node distance=1.5cm]
	\tikzstyle{every state}=[fill=white,draw=black,thick,text=black,scale=1]
	\node[state, fill=green,  opacity=.0, draw=black,thick,  text opacity=1, minimum size=0.5cm,inner sep=0pt, outer sep=0pt]  (X)  {\footnotesize};
 \node[state, fill=lightgrey,  opacity=1.0, draw=black,thick,  text opacity=1, minimum size=0.5cm,inner sep=0pt, outer sep=0pt]  (A)[below = 0.4cm of X]  {\footnotesize$A$};
	\node[state, fill=lightgrey, opacity=1.0, draw=black,thick,  text opacity=1, minimum size=0.5cm,inner sep=0pt, outer sep=0pt]    (B)[right of=A]   {\footnotesize$B$};
 \node[state, fill=green,  opacity=.0, draw=black,thick,  text opacity=1, minimum size=0.5cm,inner sep=0pt, outer sep=0pt]  (C)[below = 1.2cm of X]  {\footnotesize};
 \node[][below right = 0.1cm and -0.8cm of C] (M1) {\footnotesize \textcolor{white}{Before Tokenization }}; %{\footnotesize Before Tokenization };
 \node[][below = -0.05cm of M1] (M2) {\footnotesize \textit{Input String:} $``AABABAA"$ $\textcolor{white}{|}$};
 %\node[][below right = 1.2cm and -1.10cm of A] (M2) {\footnotesize $``AABABAAAABAAB" \rightarrow$};
	\path
	(A) edge[loop left]			node{\scriptsize$1 {-} \alpha$}	(A)
	(B) edge[bend left,below]	node{\scriptsize$\beta$}	(A)
        (A) edge[bend left,above]   node{\scriptsize$\alpha$}	(B)
        (B) edge[loop right]		node{\scriptsize$1 {-} \beta$}	(B);
	\end{tikzpicture}\hspace{-0.1cm} 
 \begin{tikzpicture}
     \node [shape=rectangle, align=center](table2) {
            \small
            \begin{tabular}{|c|c|}
            \hline
                ID & Token  \\
                \hline 
                1 &$ A$ \\
                \hline 
                2 & $B$ \\
                \hline
                3 & $AA$ \\
                \hline
            \end{tabular}
        };
        \node[][above right = -0.1cm and -2.45cm of table2] {\footnotesize Token Vocabulary};
        \node[shape=rectangle,draw=black][below = 0.25cm of table2] (bpe) {\footnotesize BPE/ MPE };
        \node[][left = 0.0cm of bpe] {\footnotesize $\longrightarrow$};
        \node[][right = 0.0cm of bpe] {\footnotesize $\longrightarrow$};
 \end{tikzpicture}\hspace{-0.1cm}
	\begin{tikzpicture}[->, >=stealth', auto, semithick]
	\tikzstyle{every state}=[fill=white,draw=black,thick,text=black,scale=1]
	\node[state, fill=maincolor2,  opacity=.3, draw=black,thick,  text opacity=1, minimum size=0.5cm,inner sep=0pt, outer sep=0pt]  (C)  {\footnotesize$AA$};
 \node[state, fill=maincolor1, opacity=.3, draw=black,thick,  text opacity=1, minimum size=0.5cm,inner sep=0pt, outer sep=0pt]    (A)[below right = 1.2cm and 0.6cm of C]   {\footnotesize$A$};
	\node[state, fill=maincolor3, opacity=.5, draw=black,thick,  text opacity=1, minimum size=0.5cm,inner sep=0pt, outer sep=0pt]    (B)[right = 1.25cm of C]   {\footnotesize$B$};
 %\node[][below right = 0.15cm and -1.5cm of A] (M1) {\footnotesize After Tokenization };
 \node[][below = -0.05cm of M1] (M2) {\footnotesize \textit{Output Tokens:} $``\textcolor{maincolor2}{AA}|\textcolor{maincolor3}{B}|\textcolor{maincolor1}{A}|\textcolor{maincolor3}{B}|\textcolor{maincolor2}{AA}"$};
	\path
	(B) edge[,left]	node{\scriptsize$\alpha\beta$}	(A)
        (A) edge[red][bend right,right]   node{\scriptsize$1.0$}	(B)
        (A) edge[red][left, right]   node[pos=0.65]{\scriptsize$0.0$}	(C)
        (A) edge[red][out=240,in=300, loop, right,right] node[pos=0.8]{\scriptsize$0.0$} (A)
        (C) edge[out=170,in=120, loop, left] node{\scriptsize${(}1{-}\alpha{)}^{2}$} (C)
        (B) edge[,below]   node{\scriptsize$(1{-}\alpha)\beta$} (C)
        (C) edge[bend right,left]   node{\scriptsize$\alpha{(}1{-}\alpha{)}$} (A)
        (C) edge[bend left,above]   node{\scriptsize$\alpha$} (B)
        (B) edge[in=10,out=60, loop, right] node{\scriptsize$1{-}\beta$}	(B);
	\end{tikzpicture}
 \vspace{-5pt}
 \captionsetup{font=footnotesize}
 \caption{Tokenization bias on a $1^{st}$-order Markov chain. Given the context token $``A"$, the model samples the next token $``B"$ with probability $1.0$ rather than $\alpha$. In practice, this bias occurs when prompts end with tokens that are part of another token, a common issue in the FIM tasks, leading to incorrect completions by the model.}   %\textcolor{red}{Explain how this relates to the FIM Task.}} 
 \label{markovchange}
 \vspace{-15pt}
\end{figure*}
%\end{document}

%% For Brandon's emacs, please do not remove:
%%% Local Variables:
%%% TeX-master: "../main"
%%% TeX-command-extra-options: "-shell-escape"
%%% End:

